Ontology Generation using Large Language Models

The ontology engineering process is complex, time-consuming, and error-prone, even for experienced ontology engineers. In this work, we investigate the potential of Large Language Models (LLMs) to provide effective OWL ontology drafts directly from ontological requirements described using user stories and competency questions. Our main contribution is the presentation and evaluation of two new prompting techniques for automated ontology development: Memoryless CQbyCQ and Ontogenia. We also emphasize the importance of three structural criteria for ontology assessment, alongside expert qualitative evaluation, highlighting the need for a multi-dimensional evaluation in order to capture the quality and usability of the generated ontologies. Our experiments, conducted on a benchmark dataset of ten ontologies with 100 distinct CQs and 29 different user stories, compare the performance of three LLMs using the two prompting techniques. The results demonstrate improvements over the current state-of-the-art in LLM-supported ontology engineering. More specifically, the model OpenAI o1-preview with Ontogenia produces ontologies of sufficient quality to meet the requirements of ontology engineers, significantly outperforming novice ontology engineers in modelling ability. However, we still note some common mistakes and variability of result quality, which is important to take into account when using LLMs for ontology authoring support. We discuss these limitations and propose directions for future research.

==> sections/limitation.tex <==
%While this study provides valuable insights, there are still avenues for future work. The first limitation concerns evaluation. Although we have included additional criteria to assess the generated ontology in greater detail, there is a need for further criteria to evaluate the and generalizability of these ontologies, along with a user-based evaluation to verify how our framework would be useful to both ontology engineers and novices. Furthermore, the ontologies produced in our study, similarly to previous research, are for the most part limited to a single module rather than being distributed across different files and modules for import and reusability. As evidenced in the Results Section \ref{sec:structural}, the model output contains repetitions, and our current approach does not prevent or eliminate extra classes or properties before their incorporation into the ontologies. 

%Our best approach for what concerns CQ coverage, Memoryless CQbyCQ, eliminates the chat history from LLMs to decrease context and improve performance. However, this approach is not suitable for other prompting techniques that heavily depend on the communication history with LLMs. The memory removal technique is only applicable to methods where each part of the ontology development can be performed independently in small parts and where there is an effective strategy for merging these partial solutions by human-in-the-loop integration.
%Furthermore, there are risks related to LLMs, similar to generative black-box methods in general. The output may contain unknown bias, leading to unexpected and undesired side effects when applying the ontologies in downstream tasks.
%Finally, challenges with the accessibility and environmental impact of LLMs, in particular GPT-4 that has been employed here, and the transparency of OpenAI's API complicate result interpretation. Overcoming these challenges is crucial for ensuring our framework is transparent and fairer. Therefore, it's clear that future research must address these issues.
This study identifies key areas for further research, highlighting the need for more robust evaluation criteria to assess the utility and generalizability of generated ontologies and advocate for additional evaluation criteria to assess generated models. Our ontologies are primarily single-module, limiting their reusability across different systems. Moreover, our methods do not adequately prevent or eliminate redundant classes or properties, as shown by model output repetitions. Our Memoryless CQbyCQ approach, which reduces context size to enhance performance, is not suitable for history-dependent modelling tasks that heavily depend on the communication history with LLMs. This technique is only applicable to methods where each part of the ontology development can be performed independently in small parts and where there is an effective strategy for merging these partial solutions by human-in-the-loop integration. Additionally, further experimentation is needed to mitigate the potential leakage effect. One way to achieve this is by applying the method to new use cases in different domains.
    %At the same time, CQs and ontology modules were not in the same file.
However, in general, using LLMs presents risks of bias, black-box LLMs affect the transparency of applications, and large models have a significant environmental impact. Addressing these challenges is essential to ensure the framework's fairness and sustainability in the future.
